GPSfM: Global Projective SFM Using Algebraic Constraints on Multi-View Fundamental Matrices

This paper addresses the problem of recovering projective camera matrices from collections of fundamental matrices in multiview settings. We make two main contributions. First, given ${n \choose 2}$ fundamental matrices computed for $n$ images, we provide a complete algebraic characterization in the form of conditions that are both necessary and sufficient to enabling the recovery of camera matrices. These conditions are based on arranging the fundamental matrices as blocks in a single matrix, called the $n$-view fundamental matrix, and characterizing this matrix in terms of the signs of its eigenvalues and rank structures. Secondly, we propose a concrete algorithm for projective structure-from-motion that utilizes this characterization. Given a complete or partial collection of measured fundamental matrices, our method seeks camera matrices that minimize a global algebraic error for the measured fundamental matrices. In contrast to existing methods, our optimization, without any initialization, produces a consistent set of fundamental matrices that corresponds to a unique set of cameras (up to a choice of projective frame). Our experiments indicate that our method achieves state of the art performance in both accuracy and running time.

==> relatedwork.tex <==

Tomasi and Kanade \cite{tomasi1992shape} have made the first step toward achieving projective reconstruction. They formulated an elegant and simple solution that uses SVD in order to to factorized the point projection matrix as a product of camera matrices and 3D point matrices. However, their method only applicable in the case of orthographic projection and require all points to be visible which is  too limited model for real data. Triggs and Strum \cite{sturm1996factorization} extended the model to perspective projection by introducing a projective depth matrix, which by multiplying in the  point projections matrix, form a rank 4 matrix.  There was several attempt to improve Triggs and Strum factorization method \cite{oliensis2007iterative,christy1996euclidean,ueshiba1998factorization,dai2013projective}, where most of them enable inclusion of missing data and improve convergence. While most of the projective factorization are global, there are a few incremental methods for projective factorization \cite{magerand2017practical,kennedy2016online,dai2013projective} which can handle outliers, missing data and bigger data set however suffer from the problems of incremental methods.\\
%In order to avoid convergence of the projective factorization into trivial %solution, Nasihatkon et al \cite{} sugested several optins how to constain %the projective depth matrix. He proposed conditions to guarantee al valid %projective reconstrution. Those conditions are known as the GRPT. \ag{check %how it relates to the var pro and then explain about var pro}\\
Methods that uses the fundamental matrices in order to initialize the bundle adjustment can have great advantage. They can have a resilience to outliers trough the fundamental matrix estimation and they can be applied on large scale scene due to independency of the points. Sweeny el al \cite{sweeney2015optimizing} first suggested an optimization scheme to improve a given viewing graph. He improves the relative geometries in the viewing graph by enforcing loop consistency constraints to the epipolar point transfer. However, his method can not be used in the full projective configuration due to dependency in self calibration and the inability to generate a projective reconstruction from a set of fundamental matrices.
Later, Sengupta et al \cite{sengupta2017new} suggested the multi-view fundamental matrix concept. He formalized the concept o-view fundamental matrix theory, however, he didn't proved sufficient conditions and moreover his method was used only as a refinement to an Euclidian method LUD \cite{ozyesil2015robust} . Hence he couldn't be used in order to perform full projective reconstruction and can be used only for refinement of Euclidean method.\\
There are several papers that consider the problem of viewing graph and its solvability \cite{levi2003viewing,rudi2010linear,ozyesil2015robust,sweeney2015optimizing}.
The viewing graph which introduced in \cite{levi2003viewing}, is   defined such that     each vertex corresponds to one out of \(n \) frames \(I_{1},..,I_n\)  and an edge between two vertices is in the graph iff there exists a calculated pairwise geometric relation    for the two corresponding frames i.e fundamental or essential matrices.  \cite{levi2003viewing,rudi2010linear}  considered minimal configurations of viewing graphs that can be solved, and reviewed  setups that can be solved linearly.    Recently \cite{trager2018solvability} has explored  more characterizations of solvable viewing graph  for general uncalibrated setup.\\  %Pairwise geometric relation between general images is defined by the  epipolar %geometry which is completely described by  the fundamental matrix, or by %the essential matrix when calibration is available.

Recently, several methods solved the problems of global Euclidean reconstruction\cite{arie2012global,ozyesil2015robust,jiang2013global,wilson2014robust}. Arie-Nachimson et al\cite{arie2012global} suggested a method that uses SDP scheme to recover rotation estimation and global linear set of equations to recover locations. Ozyesil et al \cite{ozyesil2015robust} formulated a convex relaxation to achieve robust location estimation by convex programming. His method demonstrated state of the art results in translation recovery. Jiang el al \cite{jiang2013global} formulate a global set of linear equations to solve for translation recovery.  While the global methods dominate the metric reconstruction field, to our knowledge there is no global method   to create a full projective reconstruction using only fundamental matrices. \\
Most of the methods in projective reconstruction are using rank constrained optimization scheme. Recent advancement in the field of rank optimization enable to perform accurate and efficient optimizations. Goldstein et al \cite{goldstein2014fast} has recently showed a variant of the famous ADMM model \cite{boyd2011distributed}  which accelerate the convergence of the ADMM scheme. 
 \\
\\
\\





%More robust factorization ([YDHL].. 2013 )

%Incremantal ([ppsfm] and before)

%In the calibrated case pairwise global methods are state of the art. [LUD,Mica,]
%\\Sweeney used fundamentals but must do self calibration in order to use %global approach for rotation averaging. However he assumes principle point %in the center of the image and known aspect ratio. 


